Scaling Hybrid Quantum-HPC Applications with the Quantum Framework

Hybrid quantum-high performance computing (Q-HPC) workflows are emerging as a key strategy for running quantum applications at scale in current noisy intermediate-scale quantum (NISQ) devices. These workflows must operate seamlessly across diverse simulators and hardware backends since no single simulator offers the best performance for every circuit type. Simulation efficiency depends strongly on circuit structure, entanglement, and depth, making a flexible and backend-agnostic execution model essential for fair benchmarking, informed platform selection, and ultimately the identification of quantum advantage opportunities. In this work, we extend the Quantum Framework (QFw), a modular and HPC-aware orchestration layer, to integrate multiple local backends (Qiskit Aer, NWQ-Sim, QTensor, and TN-QVM) and a cloud-based quantum backend (IonQ) under a unified interface. Using this integration, we execute a number of non-variational as well as variational workloads. The results highlight workload-specific backend advantages: while Qiskit Aer's matrix product state excels for large Ising models, NWQ-Sim not only leads on large-scale entanglement and Hamiltonian but also shows the benefits of concurrent subproblem execution in a distributed manner for optimization problems. These findings demonstrate that simulator-agnostic, HPC-aware orchestration is a practical path toward scalable, reproducible, and portable Q-HPC ecosystems, thereby accelerating progress toward demonstrating quantum advantage.

==> sections/2.3.2-background_vqls.tex <==
\subsubsection{Variational Quantum Linear Solver (VQLS)}
\label{sec:vqls}

The VQLS~\cite{Bravo_Prieto_2023} is a hybrid algorithm designed to
find the solution vector $\mathbf{x}$ to a linear system
$A\mathbf{x} = \mathbf{b}$ using near-term quantum devices.  Instead
of implementing a deep, fully quantum routine, such as the
Harrow--Hassidim--Lloyd (HHL) algorithm~\cite{Harrow_2009}, VQLS
formulates the problem as a variational optimization. A parameterized
quantum circuit (ansatz) is prepared to represent a candidate solution
$\ket{x(\boldsymbol{\theta})}$, and a cost function is defined to
quantify the residual
$\lVert A \ket{x(\boldsymbol{\theta})} - \ket{b} \rVert^2$.  The
quantum processor evaluates this cost (and, if needed, its gradient),
while a classical optimizer updates $\boldsymbol{\theta}$ to minimize
the residual. This loop continues until convergence criteria are met.

VQLS is attractive for noisy intermediate-scale quantum (NISQ) devices
because it offloads heavy numerical work to the classical optimizer
and requires relatively shallow quantum circuits. The algorithm's
modular structure allows different ansatz, measurement strategies, and
optimizers to be chosen according to hardware constraints and problem
characteristics.

Shehata \emph{et~al.}~\cite{shehata2025bridginghpcquantum}
demonstrated VQLS as a representative hybrid workload in an
HPC-quantum convergence study. Their implementation, built with the
PennyLane framework, was integrated into an HPC workflow through QFw
with minimal code changes. In this setting, each evaluation of the
cost function involved executing multiple quantum circuits, making
performance profiling and resource management critical. By leveraging
the HPC environment, the study identified optimization strategies
(e.g., choice of gradient-free optimizers) that reduced circuit counts
and improved execution time, illustrating the importance of
co-designing variational algorithms and their execution environments.

